Vision-and-Language Navigation: A Survey of Tasks, Methods, and Future Directions

A long-term goal of AI research is to build intelligent agents that can communicate with humans in natural language, perceive the environment, and perform real-world tasks. Vision-and-Language Navigation (VLN) is a fundamental and interdisciplinary research topic towards this goal, and receives increasing attention from natural language processing, computer vision, robotics, and machine learning communities. In this paper, we review contemporary studies in the emerging field of VLN, covering tasks, evaluation metrics, methods, etc. Through structured analysis of current progress and challenges, we highlight the limitations of current VLN and opportunities for future work. This paper serves as a thorough reference for the VLN research community.

==> sections/conclusion.tex <==
\section{Conclusion}

In this paper, we presented a comprehensive survey of vision-and-language navigation. We categorized the benchmarks and the methods. We also provided the current evaluation metrics and task analysis. Finally, we discussed future direction. VLN is of significant meaning and is still not well-explored. Researchers new to this area could find this paper useful due to its systematic review.

==> sections/fake-future.tex <==
\section{Discussion and Future Directions}
\label{sec:future-direction}
\xin{Use this section to discuss extensions to existing works (tasks or methods) and identify brand new future directions.}

Rather than talking about tasks development, we could also talk about how to improve task performance: causal information, knowlege graph.\xin{agree. I would use one paragraph to dicuss this. Discussion.}

\subsection{More Diverse Agents}
\xin{Discussion.}
Most agents are limited to navigating in 2D environments (sometimes indoor robots climb stairs, and there are some aerial robots), and they have minimal interaction with said environments. Another important subset of robots are robotic arms and manipulators. \citet{r2r} asked whether a robot could learn to "Bring me a Spoon". New research should ask whether a robot can learn to "Assemble that Ikea desk". 

\subsection{More Diverse Environments}
\xin{Discussion.}
Most tasks focus on very few environments: Matterport images for indoors tasks in relatively tidy home environments; and streets in major American city for outdoor tasks. Exploration on the many uncovered environments is crucial for its application. For example: warehouse or hospital settings, as well as navigating rural towns or outdoor trails.

\paragraph{Multi-Agent VLN} 
\xin{(1) multiagent is basically agent-agent collaboration, which is similar to human-robot collaboration. Merge them? (2) Use paragraph instead subsection. same for all}
Current VLN benchmarks and methods predominantly focus on tasks where only one agent navigates. However, complicated tasks in the real-world scenarios may require the collaboration of several robots. Multi-agent VLN tasks still face many obstacles in structure design, information communication, and performance evaluation.


\paragraph{Human-Robot Collaboration}
As shown in Figure~\ref{fig:relation}, VLN also studies the relationship between human and environment during navigation. In current benchmarks humans only observe the environment and act as an oracle, but do not interact with the environment. Such interaction could be crucial in reality when humans and robots are working together as teams (eg: as personal assistants or helping in construction or warehouses). This has similarities to multi-agent cooperation: in this case the agent (the human) that is changing the environment is also the oracle. 

\subsection{Simulation to Reality}

While most VLN datasets are built on photo-realistic scenes, there is still a gap in real-life robot navigation~\citep{vln-pano2real}. Real robots function in a continuous action space; meanwhile, current benchmarks usually only allow agents to "hop" through the pre-defined navigation-graph which is unrealistic for three reasons as outlined and addressed in \citet{vlnce}: the robot teleoports to nodes instead of navigating; the robot gets oracle knowledge of its exact location at all times; and the robot is given a preset list of navigable nodes which in reality it would need to determine itself. Furthermore, current VLN tasks usually do not consider real-world physics. For example, hitting a table might change its position in reality, but in current simulation environments the table would be static. Continuous implementations of realistic environments are based on image rectification, but patches of the images may be blurred or have parallax errors, making them not realistic. It would be of practical significance to build a simulation (eg: in UnReal Engine or Unity) that is both based on a 3d model (like Replica Sim) and is based on realistic imagery (like Matterport).





\subsection{Ethics and Privacy}

% The training corpus of VLN involves information from various modalities, which leads to potential hacking risk. Also, 
VLN agents that navigate indoors or outdoors would have access to personal information such as human faces. This information is usually not relevant to the task goal but will still be captured during the navigation process. Future work may explore to what extent personal information is used, whether it's stored, and how to mask personal information while still successfully training & deploying the agent.

\subsection{Multilingual and Multi-cultural}

Exploring VLN in a language other than English, or a 3D environment from diverse cultures is also a promising direction. Models developed in English may not perform well in other languages. For example, methods proposed to align the parts in instruction with current observation may not work in other languages since they have different linguistic patterns. Likewise, VLN also lacks diversity in 3D environments. For example, most outdoor VLN datasets are now using Google Street View in major American cities such as New York City, but is lacking in several developing countries. An agent trained on these datasets faces potential generalization problems in other environments.


% \paragraph{Empty Slots Explanation} For now, no datasets requires agent to actively ask for more information in natural language after given detailed route instruction. We do think it is necessary if the environment is challenging that the detailed initial instruction is not sufficient.\xin{This seems unnecessary.}
% 1. current indoor and outdoor environment, photorealistic or synthetic.

% Currently the majority of the benchmarks are about indoor environment. While the importance of outdoor navi
% Also, there is a balance between picture realness and functionality. Photo-realistic pictures captured from reality are ideal but can only be used to define tasks with pre-defined viewpoints. Synthetic environment provides a larger action space but it lacks a closer rela


==> sections/related_work.tex <==
% \section{Related Visual-and-Language Tasks}
\label{sec:related}

% VLN builds on both language and image. Here we introduce related visual-and language tasks.
% \textbf{Visual-and-Language Pre-training} has been proven effective in providing a joint representation for visual and textual modality~\citep{li2020unicoder, lu2019vilbert, tan2019lxmert}. VLN could benefit from either obtaining a good initialization or further pre-training in VLN domains. 

% \textbf{Visual Navigation} is a problem of navigating an agent from current location to find the goal target. Researchers have achieved success in both simulated environments~\citep{zhu2017target, 10.1145/3347450.3357659} and real environments~\citep{10.5555/3327144.3327168}.
% An agent in Visual Navigation tasks is usually not required to understand information from textual modality. In VLN, an agent needs to follow the given instruction and even ask for assistants in human language.

% \textbf{Embodied Question Answering (EQA)} is a AI task where an agent in a 3D environment is asked a question. Similar to VLN, the agent in EQA also navigate to explore the environment, gather information through first-person views. Instead of answering a questin in EQA, an agent in VLN is required to achieve a goal by following natural language instruction. 


==> sections/unused/anything.tex <==
\section{Methods}
\label{sec:methods}

% In Vision-and-Language Navigation, an agent interprets textual instructions and understands visual scenes to make navigation decisions. 
Many methods are proposed from different perspectives for VLN tasks. In the original setting~\citep{r2r}, the agent can not explore the test environment before executing the VLN tasks. Whether have prior access to explore the test environment or not are under different VLN setting, and we firstly introduce the prior exploration methods.

Based on the given training data and optional additional data, the VLN agents understand the vision and language information and make navigation decision each step to reach the goal target. For the methods that could be used in both settings, we categories them into Representation Learning, Action Strategy Learning, Data-Centric Learning. 

\begin{figure*}
    \centering
    \includegraphics[scale=0.35]{figures/methods.pdf}
    \caption{Categories of methods in vision-and-language navigation.}
    \label{fig:methods}
\end{figure*}

% \subsubsection{Seq-to-Seq}
% One standard backbone method used is sequence-to-sequence architecture with an attention mechanism. Many methods are built on this backbone.  
% Given natural language instruction as $x= \langle x_1,x_2,\dots\,x_L \rangle$, and the initial image observation $o_0$. The encoder takes both $x$ and $o_0$ as inputs and computes the representation $\bar{x}$. For each step $t$ in the navigation process, the decoder takes the rendered scene and the previous action $a_{t-1}$ as input and computes an distribution over the action space. 

\subsection{Prior Exploration in Test Environment}

There is a performance gap between the seen environments and unseen environments for VLN agents.
In the original setting of VLN~\citep{r2r}, the agent should be tested in an unseen environment. Meanwhile, allowing an agent to freely explore the new environment before executing tasks is also of practical benefit because it helps to adapt to a new environment such as house or apartment. Note the performance in this setting should not be directly compared with the one without prior exploration for agent evaluation purpose. Here we survey the methods for prior exploration in Test Environment. 

%The exploration on the unseen environment could either provide more supervision signal to further fine-tune the VLN agent or provide explicit knowledge guidance for the unseen environment.
\citep{fried2018speaker} explores various possible trajectories following the instruction in each session. Then they rank the exploration trajectories based on the likelihood of the instructure based on the prediction out a trained speaker model.
The exploration process could also offer more fine-tuning signal to further update the VLN model. \citet{cvpr2019wang} first introduced a matching critic measuring the compatibility between the instruction and the navigation path. For an unseen environment where no label navigation data are available and given textual instruction, the navigator is trained to follow the path the matching critic gives a high score.

Besides exploring different possible trajectories every time before starting each session, the agent could also explore once to construct a overview about the environment.
\citet{chen2021topological} proposed to build topological maps after the agent freely explored the environment. They leverages attention mechanisms to predict a navigation plan in the map and then execute the plan in action space. 
~\citet{zhou2021rethinking} considers the shortest-path route prior and regard VLN as a node classification problem after pre-exploring the environment.

\subsection{Representation Learning}

% VLN involves complex vision and language context. 
Understanding of information from both text and vision is essential for correct navigation decision. 
% Methods are also proposed to obtain a better visual representation and textual representation.
Here we introduce methods towards a better understanding of the perceived information.

\subsubsection{Pre-training}

Due to the excellent performance of the transformer-based pre-training model in various areas, it is natural to apply pre-training technology into the VLN model. Pre-training provides a relative good initialization from the knowledge in a close domain.

% The instruction in VLN tasks could be complicated and long. 
To take advantage of the natural language understanding ability of the pre-training model, \citet{li2019robust} proposed PRESS to leverage large pre-training model BERT~\citep{devlin2019bert} and GPT~\citep{radford2019language} as the encoder to improve the instruction understanding and robustness on the unseen environment. \citet{Pashevich_2021_ICCV} proposed Episodic Transformer (E.T.) that is equipped with various encoders to process different modalities. They pre-train the language encode by predicting synthetic instruction.

Visual information process also proves beneficial.
\citet{hao2020prevalent} trains a visual-textual BERT model on a large amount of image-text-action triplets from scratch to learn textual representations on VLN tasks. Their proposed PREVALENT takes image-text-action triplets as input and is trained to predict the masked tokens and the next action in a self-learning paradigm.
\citet{Qi_2021_ICCV} proposed an an
object-and-room informed sequential BERT to encode instructions and visual observations in words and object level, which strenghthen between the objects' mention and objects' visual features.

A closer relation between the pre-training task and down-stream task usually leads to a better performance. Researchers also explored pre-training on VLN task directly. By viewing VLN as a path selection problem, VLN-BERT~\citep{majumdar2020improving} pre-trains navigation model from web image-text pairs to measure the compatibility between path and instruction based on ViLBERT~\citep{NEURIPS2019_c74d97b0}.

– explicitly encoding the
inductive bias that the world is composed of objects and scenes.

VLN can be considered a partially observable Markov decision process, where the future rendered scenes are dependent on the current scene and navigation action. Meanwhile, the transformer-based pre-training model usually does not consider such interaction with the environment by design. Recurrent VLN-BERT~\citep{VLN_bert} equips a BERT pre-trained on visual-textual knowledge with a recurrent function. A BERT-structured model leverages the history representations without increasing module volume by re-using the state from the CLS token.   
Based on Recurrent VLN-BERT, \citep{moudgil2021soat} proposed a scene- and object-aware transformer (SOAT) model that uses both scene-level and object-level features.

Researchers also collected extra pre-training corpus for VLN. \citet{Guhur_2021_ICCV} collected a large-scale in-domain dataset for pre-training on vision-and-language navigation task. They further built Airbert based on the proposed dataset and achieved good performance on few-shot setting. \citet{majumdar2020improving} also proposed to use the resourceful internet contains potentially large-scale pre-training material.


\subsubsection{Graph Representation}

Objects in visual scenes and concepts in instructions has a strong logical relation. Building a graph for the relation offers a better a explicit representation for these information. 
\citet{hong2020language} proposed Language and Visual Entity Relationship Graph for modelling the
inter-modal relationships between text and vision, and the intra-modal relationships among visual entities to capture and utilize the relationships. They used a message passing algorithm for propagating information between language elements and visual entities in the graph which determines the next action to take. 
Building a graph to represent the environment also provides valuable guidance. \citet{deng-2020-evolving} introduced Evolving Graphical Planner (EGP) that constructs a graph of the navigable environment during the exploration process. The navigator reasons over the graph to select the next navigable node among action space.
\citet{vln-chasing-ghosts} proposed a mapper that constructs a semantic spatial map on-the-fly during navigation, and an end-to-end differentiable Bayes filter to identify the goal by predicting the most likely trajectory through the map according to the instructions.

\subsubsection{Memory Structure}

VLN could involve prolonged navigation steps~\citep{padmakumar2021teach, vlnce, zhu2020babywalk}. Effetively remembering and utilzing important information during the navigation history is essential for making correct decision. Toward this, various specific memory structures are proposed. 
\citet{lin2021scene} introduced a Memory-augmented attentive action decoder to help the agent to learn where to stop and what to attend to. % Scene Grounding task and Object Grounding task
\citet{nguyen-daume-iii-2019-help} proposed a memory-augmented neural agent to model decision making at a different level and an imitation learning algorithm that teaches the agent to avoid repeating past mistakes. 
\citet{zhu2020vision} proposed Cross-modal Memory Network (CMN) to remember relevant information in both textual modality and image modality. To effectively memorize information in long trajectory, \citet{chen2021history} proposed a hierarchical encoding of the
panoramic observation history 
%They restore the cross-modal experience to generate current vision representation.
%Besides, they leveraged a multi-head attention mechanism to attend to the memory about the most relevant dialogs in history.

\subsubsection{Attention Structure}

Concepts and objects that are relevant to current step decision making should receive a high attention. Various attention structures are also proposed toward a better information understanding of textual and visual modality.

\citet{landi2019embodied} employed dynamic convolutional filters to attend the visual scene and control the actions of the agent. The convolutional filters are produced via an attention mechanism and are also utilized in the scene to which the navigator moves.
\citep{zhang2020language} designed a cross-modal grounding module composed of two complementary attention mechanisms to track the correspondence between the textual and visual modalities. 
\citet{landi2020perceive} presented Perceive, Transform, and Act (PTA), where text, vision, and action are merged with a fully transformer-based model without the usage of the recurrent function.  
\citep{qi2020object} proposed Object-and-Action Aware Model (OAAM) that processes object description and direction description contained in the instruction separately.
\citet{gao2021room} proposed Room and-Object Aware Attention (ROAA) mechanism to explicitly perceive the room- and object-type information from both instruction and visual observations.

\subsubsection{Auxiliary Tasks}
A VLN environment and instruction usually contain much information that is relevant to the task goal. Therefore, except only using the signal from the navigation target, various auxiliary tasks are proposed to utilize the informative environment. 

Textual instructions in VLN may contain step-by-step guidance. The navigator needs to be aware of the navigation progress and the relation between the navigation path and instructions. \citet{cvpr2019wang} train a matching model to score the degree to which the navigation path follows instruction. The matching score is used as a reinforcement learning reward signal and a direction signal in an unseen environment. 
\citet{ma2019self} introduces Self-Monitoring navigation to estimate progress made towards the goal using vision and language co-grounding. The proposed agent identifies the correct direction by finding which part of the instruction is aligned with the current observation. The navigator leverages a progress monitor to estimate the distance between the current viewpoint and the final goal position, conditioning on navigation history and instruction.
To better utilize the rich semantic information contained in the environments, \citet{Zhu_2020_CVPR} proposed four self-supervised auxiliary reasoning tasks to help the agent to acquire knowledge of semantic representation, i.e., 1) trajectory retelling task to explain previous actions; 2) progress estimation task to evaluate the task completeness; 3) angle prediction task to predict the turn angel for next step; 4) cross-modal matching task to align the vision and the language information.
Without extra labeling cost, \citet{Huang_2019_ICCV} defines Cross-Modal Alignment to assess the fit between instruction and path, and Next Visual Scene, which predicts latent representations of future visual inputs in the path. 

\subsection{Action Strategy Learning}


VLN agents navigate a long path with many decision steps to reach the target goal. With the necessity to make decision at each step, the agents faces with tremendous navigation paths choices in a complex 3D environment. 
Here we introduce methods on the action strategy learning process.

\subsubsection{Instruction Conditioned Navigation}

\citep{kurita2020generative} introduced a generative language-grounded policy that considers available actions at each step and use Bayes' rule to obtain the posterior disctribution over actions conditioned on the natural language instruction.
The agent navigates in the environment by choosing an action that maximizes the probability of the entire instruction on a language model.


\subsubsection{Exploration during Navigation}

Exploring the environment and gathering information during the navigation process provides a clear observation of the local environment.
Beam search is a commonly used exploration strategy for finding a better trajectory~\citep{r2r, ma2019self, ma2019theregretful, tan-etal-2019-learning}. It avoids bad actions in next step by looking ahead and scoring multiple global trajectories. More sophisticated exploration strategies are also proposed toward the complexity of the VLN task.

\citet{wang2020active} developed a more active exploration module on unseen environments. The agent learns to select among visual features of different navigable views and a STOP action. The agent stops exploring and makes navigation decisions when choosing the STOP action. They further designed a recurrent network-based multi-step exploration mechanism until sufficient information was collected.  

Instead of implicitly keeping information about the environment into neural weights, Some works explicitly store the overall knowledge from exploration history. 
\citet{ke2019tactile} introduced Frontier Aware Search with backTracking (FAST). FAST combines global and local knowledge to compare partial trajectories of different lengths and backtrack when making mistakes—the agent backtrack when the progress estimator gives a low score for the current action.
\citet{ma2019theregretful} proposed Regret Module based on a progress estimator~\citep{ma2019self}. They first proposed Regret Module that decides whether to continue moving forward or roll back to a previous state. Then they introduced Progress Maker that helps to navigate according to the progress score.

\citet{Koh_2021_ICCV} designed Pathdreamer, a visual world model for indoor environment to synthesizes high-resolution visual observation along a trajectory in future viewpoints. VLN model benefits greatly from the generated observation without actual looking ahead. 

\subsubsection{Reinforcement Learning}


In reinforcement learning (RL), agents aim to maximize cumulative rewards. In this way, reinforcement learning could be brought into this Markov Decision Process (MDP).
A navigation agent interacts with the environment during the navigation process, making a decision based on the latest environment.  An increasing number of researchers have applied deep reinforcement learning to vision-and-language navigation.

\citet{cvpr2019wang} proposed a reinforced cross-modal matching (RCM) for VLN tasks that enforces cross-modal grounding both locally and globally via deep reinforcement learning. % They further introduced self-supervised imitation learning (SIL) to explore unseen environments by imitating its good decisions from the navigation history.
The real-world environment has rich dynamics. \citet{wang2018look} bridge the gap between synthetic studies and real-world practices by combining model-free and model-based reinforcement learning to predict the next state and reward. 
% The proposed Reinforced Planning Ahead (RPA) equips the VLN agent with an environment model to predict future visual perception. The agent can directly map current observation and plan the future observation simultaneously and further make action decisions based on both. 
One problem in implementing reinforcement learning into VLN is the sparsity of reward since it only receives success or fail signal at the end of the session. \citet{wang2020soft} proposed Soft Expert Distillation module to reward the agent higher when it takes action similar to expert's, and a Self Perceiving module that rewards according to the predicted navigation schedule. Distance to the target goal~\citep{roman:emnlpf20},  matching critic~\citep{cvpr2019wang, ma2019self} could also provide informative reward.
\citep{zhang2020language} proposed to recursively alternate the learning schemes of imitation and reinforcement learning to narrow the discrepancy between training and inference. Local alignment between the instructions and the landmarks could also be used as reward~\citep{landmark2021he}.

\subsubsection{Communication-based Navigation}


Being able to ask for help when uncertain about next action. Recently, researchers have also been building navigable agents that can send signal to request help or even communicate in natural language with humans for help.

\citet{roman:emnlpf20} proposed Recursive Mental Model (RMM) composed of a Questioner, a Navigator, and a Guide with three sequence-to-sequence models. 
\citet{suhr-etal-2019-executing} introduced a learning structure to distinguish recovery reasoning required for generating implicit actions and actions mentioned in regular instruction. \citet{vnla} proposed Imitation Learning with Indirect Intervention (I3L). An advisor modified the environment to influence the agent's decision in both training time and test time. 
% In the setting that the guide uses a 2D map to guide the navigator, \citet{talk_the_walk} developed Masked Attention for Spatial Convolutions (MASC) that allows for grounding utterances into the 2D overhead map in order to predict the navigator’s location.
\citet{Zhu_2021_ICCV} proposed SCoA to determine whether and what to ask help from oracle.

% Methods are also proposed for Navigation from Dialog History (NDH), a simplified task where the agent is not required to communicate with the oracle agent but only to navigate towards the goal based on dialog history. \citet{thomason:corl19} proposed using a sequence-to-sequence model with an LSTM to encode and an LSTM decoder for predicting navigation actions based on fixed ResNet embeddings of visual environment scenes. \citet{banerjee:corl20} applied the sequence-to-sequence structure with both teaching force and student forcing in a robot navigation environment. 


\subsubsection{Navigation Planning}

The navigation environment could also utlize extra task information 
The agent needs to make decision in a larger action space In continuous environment. \citep{Krantz_2021_ICCV} develops a waypoint prediction network (WPN) that predicts relative waypoints based on natural language instructions and panoramic vision. 

\citep{an2021neighbor} designed multi-module Neighbor-View Enhanced Model (NvEM) to incorporate visual contexts from neighbor views since the instruction may mention landmarks out of a single view.


%\subsection{Sim to World}


\subsection{Data-Centric Learning}

Data is an essential component in current machine learning paradigm. Vision-and-language navigation involves information from different modalities. Methods are also proposed from different aspects of the training data. 

\subsubsection{Data Augmentation}

% One of the primary challenges of the VLN task is data scarcity.
Compared with the large navigation space, complicated scenes and invariance of the textual instruction, the training data is relatively sparse. Various data augmentation methods are proposed towards the scarcity of VLN datasets.

The training set could be directly augmented via generating more path-instruction pairs from the navigable environments. \citet{fried2018speaker} trains a speaker module to generate textual instruction given navigation paths. 
% train a speaker module on ground truth path-instruction pair to generate more synthetic data. 
 The proposed speaker model could further boost the performance by ranking the path candidates during test time.   
The generated data used for augmentation could have various levels of quality. \citet{Huang_2019_ICCV} scores the cross-modal alignment to differentiate high-quality pair from low-quality pair in the data generated by~\citet{fried2018speaker}. 
\citet{huang2019multimodal} introduced a multi-modal discriminator to select valuable samples from augmented paired vision-language sequence data. They showed that a small portion of high-quality augmented data achieved similar performance with complete augmented data. 
\citet{yu2020scenic} proposed a path sampling method based on random walks to augment the training data in Room-to-Room dataset to mitigate the potential biases in the augmentation process. With the augmented data, the generalization gap between seen and unseen environments is significantly reduced.
\citet{fu2020aps} proposed an adversarial path sampler to generate challenging paths. They introduced an adversarial path sampler to select paths that are challenging for the navigator. 

Due to the rich information contained, the navigation environment itself could also be used to generate augmented data. \citet{tan-etal-2019-learning} use additional training data generated via
back-translation and visual features masking based on \citet{fried2018speaker}. They randomly mask the same visual feature in different viewpoints so that the environment is unseen to the agent to some extent. 
\citet{liu2021visionlanguage} proposed Random Environmental Mixup (REM) to split the house scenes and then to mix up to get cross-connected house scenes as augmented data. Seeing different house scenes during one navigation trip makes the agent less likely to overfit in seen houses and generalize better in unseen environments. 

Textual information in VLN may also be used for data augmentation. \citet{hong-etal-2020-sub} proposed Fine-Grained R2R dataset enrich Room-to-Room dataset with sub-instruction. They further introduced sub-instruction attention and shifting modules that sub-instructions at each time-step to use the alignment information between the instruction and the environment.

Data augmentation has proven essential in VLN tasks, and curriculum learning has been used to generate high-quality augmentation data. \citet{huang2019multimodal} used curriculum learning to train a discriminator to distinguish high-quality augmented data. They also show the efficacy of curriculum learning by extensive analysis. \citet{fu2020aps} proposed adversarial path sampler (APS) that learns to select out counter-factual augmented data. The sampler keeps learning during the selection process, and thus the selected data have a closer distribution with the original dataset. 

\citet{parvaneh2020counterfactual} intervenes in visual features to generate counterfactual trajectory via minimal edit. They improve agent’s
capabilities to generalise to new environments at test time with both training data and their counterfactuals.


\subsubsection{Curriculum Learning}

Curriculum learning~\citep{bengio2009curriculum} has received widespread attention.
The task's difficulty level is gradually increased during the training process as the model keeps improving learning ability.

BabyWalk~\citep{zhu2020babywalk} apply curriculum learning in VLN from the textual instruction perspective. Curriculum-based reinforcement learning with increasing longer instructions is leveraged to increase the language understanding ability of the VLN agent. During the training process, the instructions change from short segments of the instructions in the R2R dataset to the long instructions in the R8R dataset. 

\citep{curriculum2021zhang} rearrange the R2R dataset via regarding the room number each path covers as the sample difficulty level. self-paced curriculum learning is then adopted in VLN task. They found curriculum learning helps to smooth loss landscape and to find a better local optima.


% \subsection{External Knowledge}

\subsubsection{Multi-task Learning}

VLN shares similar modality understanding with other Vision-and-Language tasks and thus it is possible to improve both via multi-task learning. 

Visual representation model tends to overfit in seen environments. \citet{wang2020environmentagnostic} proposed an environment agnostic learning method to learn a visual representation to generalize better on unseen environments. The learning target is to build a latent representation that is invariant among the seen environment to mitigate the overfitting problem. 
\citet{ijcai2020-338} proposed attention module to train a multi-task navigation agent to follow instructions and answer questions.


\subsubsection{Sub-Instruction}

The instruction in VLN tasks provides target goals and guidance. A navigator interprets instructions in a changing environmental context.
\citet{xia2020multiview} presented LEARN FROM EVERYONE (LEO) to leverage multiple instructions for the same trajectory. Each instruction provides a different angle to describe the trajectory, and LEO encodes all the instructions with a shared set of parameters.   
Instruction could be long and complicated. To better understand the relation between the visual scenes during navigation with all parts of the given instruction, \citet{hong-etal-2020-sub} splits the long instruction in the R2R dataset into short sub-instructions and align the sub-instructions with visual sequences. With the enhanced sub-instructions, the agent is provided with more detailed supervision from a language perspective. They further train a sub-instruction selection model to focus on important sub-instruction.



% \subsubsection{Extra Environment Signal}



\eliana{\section{Future Directions (Eliana editing...)}}
\label{sec:future-direction}

\subsection{Deploying from Simulation to Real}
\subsubsection{More Realistic Image Synthesis}
\eliana{While several simulators use both real data and synthetic data (Matterport3D, Gibson, Replica, Habitat, RoboTHOR, VLN-CE), there is still a gap in real life robot navigation~\citep{vln-pano2real}. Countless movies have used synthetic imagery (eg: UnReal Engine) that is near-indistinguishable from reality. However, the photo-realistic simulations are noisy, because they are using holographic transforms to minic to motion of a robot through discrete (and sparse) panoramic images. This results in occlusion, grainy patches, and bad parallax. A direction to explore would be creating 3D environments in more powerful simulation engines (Unity or UnrealEngine) so that a simulation is more representative of real-world perception. }

\subsubsection{Removing the Nav-Graph}
\Qi{Instead of removing the Nav-Graph, we can also predict Nav-Graph in the continues environments. There are many benefits of nav-graph (for example, easy to train a navigator). We can't simply remove it.}\xin{I agree with Qi. Also, the page limit is 8 and we will probably use 1 page for discussion and future directions. That said, we cannot use half page to discuss sim-to-real transfer. Each future direction (e.g., sim-to-real transfer, multi-agent VLN) should be discussed using one paragraph concisely. }
\eliana{Most benchmarks usually only allow agents to navigate through the pre-defined nav-graph. This artificially gives the agent a priori information as to where it can possibly navigate to, gives it perfect localization, and teleportation. These problems are addresses in Jacob Krantz's 2020 paper. More reserach outside the navigation graph will greatly help agents navigate in continuous actions spaces, as discussed in the section below. }

\subsubsection{Continuous Action Spaces}
\eliana{While normally these VLN agents output one discrete actions (turn 15 deg left / right/ go forward 0.25[m]  / stop), a robot lives in a continuous action-space. It can rotate a continuous amount, drive forward a continuous amount, and do both at the same time to follow an arc (drive forward while turning). While more complex of a trajectory, it allows the robot to move more fluidly through the environment.}

\subsection{Multi-Agent VLN}
\eliana{Current VLN benchmarks and methods mainly focus on tasks where only one agent is required to navigate. However, complicated tasks in the real world may require the collaboration of several robots. Multi-agent VLN tasks still face many obstacles in structure design, information communication, and performance evaluation.}

Data scarcity is a common problem, and various data augmentation methods have been proven helpful in general VLN tasks. However, data augmentation could be costly, especially for high-quality data. Meanwhile, there are abundant raw data on text, image, and generation navigation area. Successful adaptation into the VLN domain could lead to a tremendous performance boost.\par

==> tables/not-used-table.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{c|cccc}
        \toprule
         \textbf{Level} & \textbf{Name} & \textbf{Simulator} & \textbf{Language-Active} & Environment \\
         \midrule
         \multirow{5}{*}{Level 1} & Room-to-Room~\citep{r2r} & Matterport3D & \xmark  & Indoor\\
         & Room-for-Room~\citep{jain-etal-2019-stay} & Matterport3D & \xmark  & Indoor\\
         & R6R, R8R~\citep{zhu2020babywalk} & Matterport3D & \xmark  & Indoor\\
         & Room-Across-Room~\citep{rxr} & Matterport3D  & \xmark  & Indoor\\
         & XL-R2R~\citep{yan2020crosslingual} & Matterport3D & \xmark  & Indoor\\
         & VLNCE~\citep{vlnce} & Habitat & \xmark  & Indoor\\
         & StreetLearn~\citep{mirowski2019streetlearn} & Google Street View & \xmark & Outdoor\\
         & StreetNav~\citep{hermann2020learning} & Google Street View & \xmark & Outdoor\\
         & TOUCHDOWN~\citep{touchdown} & Google Street View & \xmark & Outdoor\\
         & Talk2Nav~\citep{vasudevan2021talk2nav} & Google Street View & \xmark & Outdoor\\
         \midrule
         
         \multirow{2}{*}{Level 2} & RoomNav~\citep{wu2018building} & House3D & \xmark & Indoor\\
         & REVERIE~\citep{reverie} & Matterport3D & \xmark & Indoor\\
         & SOON~\citep{zhu2021soon} & Matterport3D & \xmark & Indoor\\
         \midrule

         \multirow{1}{*}{Level 3} & ALFRED~\citep{alfred} & AI2-THOR & \xmark & Indoor\\
         \midrule

         \multirow{2}{*}{Level 4} & VNLA~\citep{vnla} & Matterport3D & \cmark & Indoor\\
         & HANNA~\citep{nguyen-daume-iii-2019-help} & Matterport3D & \cmark & Indoor\\
         & CEREALBAR~\citep{suhr-etal-2019-executing} & - & \cmark & Indoor\\
         & Just Ask~\citep{chi2020just} & Matterport3D & \cmark & Indoor\\
         & CVDN~\citep{thomason:corl19} & Matterport3D & \cmark & Indoor\\
         & NDH~\citep{thomason:corl19} & Matterport3D & \xmark & Indoor\\
         & RobotSlang~\citep{banerjee:corl20} & - & \cmark & Indoor\\
         & Talk the Walk~\citep{talk_the_walk} & - & \cmark & Outdoor\\
         & TEACh~\citep{padmakumar2021teach} & AI2-THOR & \cmark & Indoor \\


         \bottomrule
    \end{tabular}
    \caption{Vision-and-Language Navigation datasets. Language-Active means the agent needs to use natural language for help.}
    \label{tab:my_label}
\end{table*}

% could add Photorealistic and continuous



\noindent
\begin{table*}[]
    \centering
    \begin{tabular}{|l||*{3}{c|}}
    \hline
    \backslashbox{Instruction}{Interaction}
    &\makebox[9em]{No Interaction}&\makebox[9em]{Guidance}&\makebox[9em]{Communication}\\\hline\hline
    Fine-grained Navigation &&&\\\hline
    Coarse Navigation &&&\\\hline
    Nav + x &&&\\\hline
    \end{tabular}
    \caption{Vision-and-Language Navigation datasets. Language-Active means the agent needs to use natural language for help.}
    \label{tab:my_label}
\end{table*}


\noindent
\begin{table*}[]
    \centering
    \begin{tabular}{|l||*{3}{c|}}
    \hline
    \backslashbox{Instruction}{Interaction}&\makebox[9em]{Fine-grained Navigation} & \makebox[9em]{Coarse Navigation} & \makebox[9em]{Nav + Manipulation}\\\hline\hline
    No Interaction &Room-to-Room~\citep{r2r} TOUCHDOWN~\citep{touchdown} & REVERIE~\citep{reverie} RoomNav~\citep{wu2018building} & ALFRED~\citep{alfred}  \\\hline
    Guidance & &&\\\hline
    Communication &&&\\\hline
    \end{tabular}
    \caption{Vision-and-Language Navigation datasets.}
    \label{tab:my_label}
\end{table*}



\noindent
\begin{table*}[]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{|l||p{12em}|p{12em}|p{9em}|}
    \hline
    \backslashbox{Interation \\ w/ Oracle}{Task \\ Complexity}& Route-Detailed & Object-Targeting & Navigation + Manipulation\\\hline\hline
    No Interaction & \small{*Matterport3D group;\newline *Google Street View Group; LANI~\citep{misra2018mapping}} & \small{REVERIE~\citep{reverie}; RoomNav~\citep{wu2018building}; SOON~\citep{zhu2021soon}} & \small{ALFRED~\citep{alfred}}  \\\hline
    
    Guidance Only & \small{Just Ask~\citep{chi2020just}} & \small{VNLA~\citep{vnla}; HANNA~\citep{nguyen-daume-iii-2019-help}; CEREALBAR~\citep{suhr-etal-2019-executing}} & -\\\hline
    
    Dialog & - & \small{CVDN~\citep{thomason:corl19}; RobotSlang~\citep{banerjee:corl20}; Talk the Walk~\citep{talk_the_walk}} & \small{TEACh~\citep{padmakumar2021teach}} \\\hline
    \end{tabular}}
    \caption{Vision-and-Language Navigation datasets. *Matterport3D group includes Room-to-Room~\citep{r2r}, Room-for-Room~\citep{jain-etal-2019-stay}, R6R, R8R~\citep{zhu2020babywalk}, Room-Across-Room~\citep{rxr}, XL-R2R~\citep{yan2020crosslingual}, VLNCE~\citep{vlnce}. *Google Street View includes StreetLearn~\citep{mirowski2019streetlearn}; StreetNav~\citep{hermann2020learning}, TOUCHDOWN~\citep{touchdown} \newline Talk2Nav~\citep{vasudevan2021talk2nav}. }
    \label{tab:my_label}
\end{table*}

